Simultaneous Information and Energy Transmission with Short Packets and Finite Constellations

This paper characterizes the trade-offs between information and energy transmission over an additive white Gaussian noise channel in the finite block-length regime with finite channel input symbols. These trade-offs are characterized in the form of inequalities involving the information transmission rate, energy transmission rate, decoding error probability (DEP) and energy outage probability (EOP) for a given finite block-length code. The first set of results identify the set of necessary conditions that a given code must satisfy for simultaneous information and energy transmission. Following this, a novel method for constructing a family of codes that can satisfy a target information rate, energy rate, DEP and EOP is proposed. Finally, the achievability results identify the set of tuples of information rate, energy rate, DEP and EOP that can be simultaneously achieved by the constructed family of codes.

==> BackUp1-Introduction-Perlaza.tex <==
\section{Introduction} \label{sec:intro}
Simultaneous information and energy transmission (SIET) (also known as simultaneous wireless information and power transfer (SWIPT)) employs radio frequency (RF) signals to simultaneously accomplish the tasks of conveying information and providing energy to (possibly different) devices.
% In the following, for the sake of correctness, the denomination ``energy transmission'' is preferred against ``power transfer'', and thus, the acronym SIET is adopted in the remainder of this paper. 
A fundamental issue of interest in SIET is, to characterize the fundamental limits on the information rate, energy rate, decoding error probability (DEP) and energy outage probability (EOP) achievable by a given code and to study the trade-offs between these parameters.
The trade-offs between information and energy transmission rates in SIET have previously been studied in the asymptotic regime~\cite{varshney2008transporting,amor2016fundamental,NizarItw2021,GroverSahai,amor2016feedback,KhalfetGIC} where the assumption of infinitely long transmissions guarantees that the DEP and the EOP can be made arbitrarily close to zero. Thus, the focus of the asymptotic results is only on the information and energy transmission rates. In the finite block-length regime, however, the DEP and EOP are bounded away from zero and pose additional constraints on the fundamental limits of SIET. 
%These questions have previously been answered in the asymptotic regime where the assumption of infinitely long transmissions guarantees that the decoding error probability (DEP) and the energy outage probability (EOP) can be made arbitrarily close to zero, and thus, the focus is only on the information and energy transmission rates. In the finite block-length regime, however, the DEP and EOP are bounded away from zero and pose additional constraints on the fundamental limits of SIET. 
%However, the consideration of finite block-lengths brings into action
% It is of particular interest to determine the fundamental limits of SIET 

A common assumption in the study of SIET over an additive white Gaussian noise (AWGN) channel is that the channel inputs are derived independently from a Gaussian distribution.
In a departure from this norm, this work considers the more practical, discrete set of channel input symbols.
Unlike Gaussian inputs, the bounds obtained for finite discrete sets of channel input symbols provide insights for practical systems that operate with finite block-lengths and finite sets of channel inputs. 
In this work, all the parameters of concern, namely, the energy transmission rate, the information transmission rate, DEP and EOP are evaluated as a function of the type.
A type is understood in the sense of  the empirical frequency with which each channel input symbol appears in the codewords~\cite{CsiszarMoT}.

\subsection{State of the art}
The existing body of work in SIET can be studied under three main categories. The first is the study of the the trade-offs between the information and energy rates that can be simultaneously transmitted by an RF signal.  
Earlier research in this area is focused primarily on the asymptotic regime~\cite{varshney2008transporting,GroverSahai,amor2016fundamental, NizarItw2021}. In this case, the notion of the information-energy region generalizes to the set of all information and energy rate tuples that can be simultaneously achieved in the asymptotic block-length regime~\cite{amor2016fundamental}. To capture the trade-off between the information and energy rates,~\cite{varshney2008transporting} defines a capacity-energy function for various channels including the discrete memoryless channel, binary symmetric channel, and the AWGN channel. In~\cite{GroverSahai}, the information-energy trade-off is studied for a coupled-inductor circuit that models a  slow frequency-selective fading channel.
The information-energy capacity region of the Gaussian multiple access channel is characterized in~\cite{amor2016feedback,amor2017feedback}, whereas the information-energy capacity region of the Gaussian interference channel is approximated in~\cite{KhalfetGIC}. Nonetheless, the information-energy trade-off is not the only trade-off involved in SIET. In the finite block-length regime, several other trade-offs appear (between the information rate, energy rate, DEP and EOP) which are taken into consideration in this paper. Within the finite block-length regime,~\cite{perlaza2018simultaneous} and~\cite{khalfet2019ultra} provide a characterization of the information-energy capacity region with binary antipodal channel inputs. 
Converse and achievability bounds on SIET for a given arbitrary number of channel inputs is presented in~\cite{zuhraITW} and~\cite{zuhraISIT}, respectively. % {Re-phrase so it doesn't seem like everything has already been done in these }
%It has been shown in~\cite{zuhraITW} and~\cite{zuhraISIT} that, in the non-asymptotic regime, these limits are a function of the type induced by the code used for the transmission. 
The impact of energy harvester non-linearities on the fundamental limits of SIET in the finite block-length regime has been studied in~\cite{zuhraITW2}.

%The earlier research into the information-energy trade-offs in SIET focus on the asymptotic regime~\cite{varshney2008transporting,GroverSahai,amor2016fundamental, NizarItw2021,6373669}. In this case, the notion of information-energy region generalizes to the set of all information and energy rate tuples that can be simultaneously achieved in the asymptotic block-length regime~\cite{amor2016fundamental}. To capture the trade-off between the information and energy rates,~\cite{varshney2008transporting} defines a capacity-energy function for various channels including the discrete memoryless channel, binary noiseless channel, binary symmetric channel, Z-channel and the AWGN channel. In~\cite{GroverSahai}, the information-energy trade-off is studied for a coupled-inductor circuit that models a  slow frequency-selective fading channel.
%The information-energy capacity region of the Gaussian multiple access channel is characterized in~\cite{amor2016feedback}, whereas the information-energy capacity region of the Gaussian interference channel is approximated in~\cite{KhalfetGIC}. Nonetheless, the information-energy trade-off is not the only trade-off involved in SIET. In the finite block-length regime, several other trade-offs appear which are taken into consideration in this paper.

The second area of research that has received considerable attention in SIET is the modeling of the energy harvester (EH) circuits with the aim of providing accurate estimates of the energy harevested from an RF signal. This line of inquiry has revealed that, due to the presence of non-linear elements such as diodes in the EH circuits, the expected energy harvested from a signal is a function of the fourth power of the signal magnitude~\cite{varasteh2017wireless} in addition to the squared magnitude as was conventionally assumed (see~\cite{amor2016fundamental}, \cite{amor2016feedback} and~\cite{khalfet2019ultra}). Recent research on EH non-linearities~\cite{8115220,7547357} has shown that energy models that do not account for these non-linearities result in inaccurate estimates of the harvested energy. This work accounts for the EH non-linearities by adopting the models proposed in the literature for determining the energy harvested from the transmitted RF signals. 

The third category of research deals with aspects related to the design and implementation of SIET such as signal and system design, resource allocation, receiver architectures, energy harvester circuits, and decoding strategies. Optimal waveform design for SIET from a multi-antenna transmitter to multiple single antenna receivers is studied in~\cite{9447959}. Signal and system design exclusively for wireless energy transmission has been studied in~\cite{7547357,9411899,9184149,7867826, 9447237} and~\cite{9153166}. In~\cite{9377479}, the authors optimize resource allocation and beamforming for intelligent reflecting surfaces aided SIET. The memory of non-linear elements in the EH circuit is modeled as a Markov decision process in~\cite{9241856} and a learning based model is proposed for the EH circuit.
 An algorithm for designing a circular quadrature amplitude modulation scheme for SIET that maximizes the peak-to-average power ratio has been proposed in~\cite{9593249}. This paper contributes to this line of research by providing a method of code construction for SIET that satisfies a given feasible tuple of information rate, energy rate, DEP and EOP. 
 
More comprehensive overviews of the work on SIET in the second and third categories detailed above, can be found in~\cite{survey,surveyA},~\cite{8476597}, and~\cite{ClerckxFoundations}. A comparison of relevant aspects of the existing literature on SIET with this work is provided in Table~\ref{TableSOA} below. A tick mark indicates that the specific factor has been taken into consideration in the paper while a dash indicates that the concerned feature has not been taken into consideration in that reference.

\begin{table*}[t] 
\captionof{table}{Summary of the state-of-art} 
\centering
\begin{tabular}{ | m{1.5 cm} | m{1.3 cm} |m{1.7 cm} |m{1.5 cm} | m{3cm}| m{1cm}| m{1cm}|} 
% \hline
%& \multicolumn{5}{c}{\textbf{Point-to-point}}&\\
 \hline
  \textbf{Reference}  & \textbf{Channel inputs} & \textbf{Block-length} & \textbf{EH non-linearities} & \textbf{Channel} & \textbf{DEP} & \textbf{EOP} \\
 \hline
 \hline
\cite{varshney2008transporting}       & Infinite                    & Asymptotic			& -				& DMC, AWGN & - & -\\
\hline
\cite{GroverSahai}  		      &Infinite			 & 	Asymptotic			& 	-			&  AWGN + Frequency-selective fading & - & - \\
\hline
\cite{NizarItw2021} 			& Infinite                    &     Asymptotic                            & \checkmark 		& Rayleigh fading & - & - \\
\hline
\cite{6373669} 				& Infinite 	               & Asymptotic				& 	-			& Flat fading & - & - \\
\hline
\cite{9241856} 		                & Infinite		       	       & Asymptotic		& -				& AWGN& - & - \\
 \hline
 \cite{9149424} 		        & Finite		       	       & 	Asymptotic			& -				& AWGN + Fading& - & - \\
 \hline
 \cite{9377479} 		        & Finite		       	       & 	Asymptotic			& -				& AWGN + Flat-fading& - & - \\
 \hline
 \cite{7998252} 		        & Finite		       	              & -			& 	-			& AWGN + Rayleigh fading & \checkmark & - \\
 \hline
  \cite{9593249} 		& Finite		       	              & -			& -				& AWGN& -  & - \\
 \hline
    \cite{varasteh2017wireless} 	& Infinite		       	              & Asymptotic	& \checkmark			& AWGN& - & - \\
 \hline
     \cite{8115220} 		        & Infinite		       	              & Asymptotic	& \checkmark			& Multi-path fading & - & - \\
     \hline
   \cite{9741251}			&	Uncountable	&	Asymptotic	&	-		&	AWGN + Rayleigh fading	& \checkmark & -\\
  \hline
   \cite{9734045}			&	Uncountable	&	Asymptotic	& -		&	AWGN + Rayleigh and Rician fading	& - & - \\
  \hline
   \cite{liu2022joint}			&	Uncountable	&	Asymptotic	&	-		&	AWGN	& -& -\\
   \hline
   \cite{9502719}			&	Uncountable	&	Asymptotic	&	\checkmark		&	Multi-path fading	& - & -\\     
 \hline
    \cite{6489506}			&	Uncountable	&	Asymptotic	&	-		&	Multi-path fading	& - & -\\     
 \hline
     \cite{ 7063588}			&	Uncountable	&	Asymptotic	&	-		&	AWGN + Flat-fading	& - & -\\     
 \hline
      \cite{9169700 }			&	Finite	&	Finite	&	 \checkmark			&	AWGN 	& - & -\\     
 \hline
  \cite{perlaza2018simultaneous}               & Finite                         & Finite              & 	-			& BSC & \checkmark & \checkmark\\
\hline
 \cite{khalfet2019ultra} 	& Finite		       	              & Finite			& 	-			& BSC& - & -\\
 \hline
      \textbf{This work} 	& Finite		       	              & Finite	& \checkmark			& AWGN& \checkmark & \checkmark\\
        \hline
%  \hline
  % MAC starts here:
%& \multicolumn{5}{c}{\textbf{MAC}}&\\
% \hline
% \cite{amor2016feedback} 		& Finite		       	       & Asymptotic				& -	& AWGN& - & -\\
% \hline
% \cite{KhalfetGIC} 		        & Finite		       	       & Asymptotic				&   -    &Gaussian interference& - & -\\
% \hline
%      \cite{9743404}			&	Uncountable	&	Asymptotic	& -		&	Path-loss, Rayleigh fading	& \checkmark & \checkmark\\
% \hline
%        \cite{9743923}			&	Uncountable	&	Asymptotic	&	\checkmark		&	AWGN	& - & -\\
%  \hline
%   \cite{8078258}			&	Uncountable	&	Asymptotic	&	-		&	AWGN + flat fading	& \checkmark & \checkmark\\     
%    \hline
%    \cite{9133435}			&	Uncountable	&	Asymptotic	&	-		&	AWGN + flat fading	& - & -\\      
%    \hline
%        \cite{6571308}			&	Uncountable	&	Asymptotic	&	-		&	AWGN + flat fading	& - & -\\      
%    \hline
 \end{tabular} \label{TableSOA}
 \end{table*}

\subsection{Contributions}
This work studies the trade-offs involved in the joint transmission of information and energy in the finite block-length regime for a given finite and discrete set of channel input symbols (\ie, constellations, such as QPSK, 16-QAM, 64-QAM etc).
% In the current literature, no techniques exist for analyzing such a setup. 
% The analysis in this work breaks away from the traditional method of taking a DEP and then bounding the information rate in terms of the DEP. 
% Instead, this work evaluates the trade-offs between the energy transmission rate, the information transmission rate, DEP and EOP for a given codebook.
% This problem setting follows a similar vein to the problem of characterizing the fundamental limits of a multiple-access channel with finite input and output alphabets and finite block-lengths under mismatched decoding treated in~\cite{Lapidoth1996}.
% Under mismatched decoding, trade-offs emerge between the DEP, information transmission rate and the block-length which have been studied in~\cite{scarlett2020information}.
The main contributions are summarized below.
\todo{Update contributions}
\begin{itemize}
% \item A \note{new technique} for analyzing the \note{fundamental limits} of SIET in the finite block-length regime with finite and discrete set of channel inputs is developed using the method of types~\cite{CsiszarMoT}. It is shown that the bounds on all the parameters of SIET can be expressed as a function of the type induced by the code. Therefore, the trade-offs between these parameters can be controlled by adjusting the type. 

% It is noteworthy that though this technique is developed in the context of SIET, its applicability is not limited to SIET. The technique   provides an elegant method of defining the fundamental limits in any information theoretic problem where the parameters under consideration can be expressed as a function of the type induced by the code.
\item Impossibility bounds for finite block-length SIET over an AWGN channel with a peak-amplitude constraint are characterized for a given finite set of channel input symbols.
These bounds define the set of information rate, energy rate, DEP and EOP tuples that cannot be simultaneously achieved by any code that employs the given set of channel input symbols. 
\item Based on the insights provided by the impossibility results, a method of constructing codes for SIET over an AWGN channel in the finite block-length regime is proposed that can meet the given requirements of information and energy transmission simultaneously.
\item Achievability results are provided for the constructed family of codes. 
These results characterize the set of information rate, energy rate, DEP and EOP tuples that can be simultaneously achieved by at least one code from the constructed family of codes.
\item The trade-offs between the information rate, energy rate, DEP and EOP are illustrated through various instructive examples.
The information-energy region is also illustrated for a given set of channel input symbols.
% The study of the gaps between the impossibility and achievability results shows that the bounds match in terms of the information rate, the energy rate and the EOP. 
% However, owing to the choice of the decoding regions made during the construction, for a given information rate, energy rate and EOP, the achieved DEP is higher than the impossibility bound.
\end{itemize}

The following subsection summarizes the important notation used in this paper.
  
\subsection{Notation} \label{SecNotation}
The sets of natural, real and complex numbers are denoted by $\ints$, $\reals$ and $\complex$, respectively. In particular, $0 \notin \ints$.
%The Borel $\sigma$-algebra on $\reals$ is denoted by $\mathscr{B}(\reals)$.
Random variables and random vectors are denoted by uppercase letters and uppercase bold letters, respectively. Scalars are denoted by lowercase letters and vectors by lowercase bold letters. The real and imaginary parts of a complex number $c \in \complex$ are denoted by  $\Re(c)$ and $\Im(c)$, respectively. The complex conjugate of $c \in \complex$ is denoted by $c^\star$ and the magnitude of $c$ is denoted by $|c|$.  The imaginary unit is denoted by $\mathrm{i}$, \ie, $\mathrm{i}^2 = -1$.  
%The Kullback-Leibler (KL) divergence between two measures $P$ and $R$, with $P$ absolutely continuous with $R$, is denoted by $D(P||R)  = \int \log \frac{\mathrm{d}P}{\mathrm{d}R} \mathrm{d}P$, where $\frac{\mathrm{d}P}{\mathrm{d}R}$ denotes the Radon-Nykodim derivative of $P$ with respect to~$R$. 
The empty set is denoted by $\phi$. The $\sinc$ function is defined as follows
\begin{IEEEeqnarray}{rCl} \label{EqSinc}
\sinc(t) \triangleq \frac{\sin(\pi t)}{\pi t},
\end{IEEEeqnarray}
and the $\mathrm{Q}$ function is given by the following:
\begin{IEEEeqnarray}{rCl} \label{DefQfunc}
\mathrm{Q}(x) = \int_x^\infty \frac{1}{\sqrt{2 \pi}} \exp \left(-\frac{t^2}{2} \right) \mathrm{d}t.
\end{IEEEeqnarray}
%
The rest of this paper is organized as follows.
The system model is presented in Section~\ref{sec:system_model}.
The \note{necessary conditions on the parameters of} finite block-length codes for SIET are characterized in Section~\ref{sec:results}. Section~\ref{SecAchievability} provides the construction of codes for finite block-length SIET followed by the characterization of an achievable region.
The trade-offs between various parameters of finite block-length SIET are elucidated using various examples in Section~\ref{SecDiscussion}. 
% Section~\ref{SecDiscussion} also provides a comparison of the proposed bounds with the existing state of the art.\clearpage
 \appendix
 \input{impossibility_proofs}
 \input{lemmas_achievability}
 \input{misc_lemmas_dep}
 \input{appendix.tex}
 
%\section{Biography Section}
%If you have an EPS/PDF photo (graphicx package needed), extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
% your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
% simpler here.)c
% 
%\vspace{11pt}
%
%\bf{If you include a photo:}\vspace{-33pt}
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
%Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
%Use the author name as the 3rd argument followed by the biography text.
%\end{IEEEbiography}
%
%\vspace{11pt}
%
%\bf{If you will not include a photo:}\vspace{-33pt}
%\begin{IEEEbiographynophoto}{John Doe}
%Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
%\end{IEEEbiographynophoto}
%
%
%
%
%\vfill

\end{document}



